SMUG: Towards robust MRI reconstruction by smoothed unrolling

Although deep learning (DL) has gained much popularity for accelerated magnetic resonance imaging (MRI), recent studies have shown that DL-based MRI reconstruction models could be oversensitive to tiny input perturbations (that are called 'adversarial perturbations'), which cause unstable, low-quality reconstructed images. This raises the question of how to design robust DL methods for MRI reconstruction. To address this problem, we propose a novel image reconstruction framework, termed SMOOTHED UNROLLING (SMUG), which advances a deep unrolling-based MRI reconstruction model using a randomized smoothing (RS)-based robust learning operation. RS, which improves the tolerance of a model against input noises, has been widely used in the design of adversarial defense for image classification. Yet, we find that the conventional design that applies RS to the entire DL process is ineffective for MRI reconstruction. We show that SMUG addresses the above issue by customizing the RS operation based on the unrolling architecture of the DL-based MRI reconstruction model. Compared to the vanilla RS approach and several variants of SMUG, we show that SMUG improves the robustness of MRI reconstruction with respect to a diverse set of perturbation sources, including perturbations to the input measurements, different measurement sampling rates, and different unrolling steps. Code for SMUG will be available at https://github.com/LGM70/SMUG.

==> sections_old/sec_method.tex <==
\section{{\us}: SMoothed UnrollinG}
\label{sec: approach}

In this section, we describe our proposed {\us} method, in which we integrate {\modl} \cite{aggarwal2018modl} with randomized smoothing \cite{cohen2019certified}, to solve the instability problems mentioned in Sec. \ref{sec: preliminaries}. We first explicitly describe the architecture of our {\us} method in Sec. \ref{sec: unrolling}. Later, we elaborate on our training scheme in Sec. \ref{sec: how to smoothing}.

\subsection{Unrolling: key in smoothing on MoDL}
\label{sec: unrolling}

Following the denoised smoothing \cite{salman2020denoised}, we use a custom-trained denoiser to make the base model, \textit{i.e.} {\modl}, robust to Gaussian noise before applying randomized smoothing to generate robustness against adversarial perturbations. But instead of introducing a new denoiser, we exploit the denoiser in {\modl} for model simplicity and overall time efficiency. Compared to appending a new denoiser, our approach of reusing the existing denoiser in {\modl} is capable of removing Gaussian noises in every unrolling step, which enhances the Gaussian noise robustness of the base model and makes it more potential for randomized smoothing.

We then apply randomized smoothing \cite{cohen2019certified} to {\modl}. 
We present two smoothing architectures here: 1) {\us} on the whole ({\us} ($\cD + \mathcal{DC}$)), and 2) {\us}. {\us} is proposed to integrate randomized smoothing with {\modl} naturally. The differences between these architectures and \ref{eq: denoised smoothing mri} mainly focus on where to add the Gaussian noises and where to take the majority vote, \textit{i.e.} estimate the expectation in MRI reconstruction. Their comparison can also be seen in Fig. \ref{fig: model-arch}.
In \ref{eq: denoised smoothing mri}, the Gaussian noises $\epsilon$ are added on the input of the entire {\modl}, $\bx_0$, and the expectation \textit{w.r.t.} $\epsilon$ is estimated on the output of the entire {\modl}, $\bx_K$. In {\us}, however, the Gaussian noises $\epsilon$ are added on the input of \textit{every} unrolling step in {\modl}, $\bx_k$, and the expectations are estimated in \textit{every} unrolling step on the output of the whole unrolling step, \textit{i.e.} the output of the $\mathcal{DC}$, for {\us} on the whole, and the output of the denoiser for {\us}. 

\begin{figure}[htb]
% \vspace*{-3mm}
    \centering
    \begin{subfigure}{.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/E2E_Smoothing.pdf}
        \caption{\footnotesize{\ref{eq: denoised smoothing mri}
        }}
    \end{subfigure}
    
    \begin{subfigure}{.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/SMUG_whole.pdf}
        \caption{\footnotesize{{\us} on the whole
        }}
    \end{subfigure}

    \begin{subfigure}{.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/SMUG.pdf}
        \caption{\footnotesize{\us}}
    \end{subfigure}
    
    \vspace*{-1em}
    \caption{\footnotesize{The architecture of (a) \ref{eq: denoised smoothing mri}, (b) {\us} on the whole, and (c) {\us}.}}
    \label{fig: model-arch}
    % \vspace*{-4mm}
\end{figure}

% To be congruent with the presence of the denoiser in every unrolling step, we adopt an unrolling version of randomized smoothing, which we call {\us}. {\us} exploits the full potential of the unrolling presence of the denoiser in Gaussian noise robustness, thus obtaining high robustness for {\modl}. 

More concretely, our method of {\us} can be formularized as the following iterative algorithm, 
\begin{subequations}
\label{eq: unrolling smoothing}
\begin{align}
    \bz_k &= \mathbb{E}_{\epsilon\sim\mathcal{N}(0,\sigma^2I)} \cD(\bm{\theta}; \bx_k + \epsilon)
    \\
    \bx_{k+1} &=\underset{\bx}{\arg\min} \sum_{c=1}^{N_c}||A_c \bx - \by_c||_2^2 + \lambda ||\bx-\bz_k||^2
    \label{eq: unrolling smoothing optimization}
\end{align}
\end{subequations}
which is initialized with $\bx_0=A^H\by$, where $A^H$ transforms k-space data to the image domain. $\bz_k$ is estimated through the Monte Carlo sampling. In every unrolling step (\textit{i.e.} iteration), we first generate a number of Gaussian noises $\epsilon \sim \mathcal N(0, \sigma I^2)$, and add it to $\bx_k$. Then, we estimate the expectation of the denoised version of these images.
The denoiser $\cD (\cdot)$ is different from that in {\modl}, because the denoiser here is custom-trained to remove the Gaussian noises as well as alias artifacts and noises obtained in the undersampling and the upstream image processing. 
Finally, the conjugate gradient method is used to solve the optimization problem \eqref{eq: unrolling smoothing optimization}.


We evaluate the effectiveness of the three architectures towards adversarial robustness, and the results are shown in Table \ref{tab: exp_smoothing} and Fig. \ref{fig:archi_PSNR}. Experiment shows that {\us} has the highest robustness and comparable accuracy with other models. This implies the effectiveness of our proposed {\us}. We suspect that {\us} exploits the full potential of the presence of denoiser in each unrolling step compared to \ref{eq: denoised smoothing mri}, and avoids the noises introduced by the conjugate gradient method compared to {\us} on the whole.

\subsection{Unrolling loss}
\label{sec: how to smoothing}

The effectiveness of {\us} highly depends on the training scheme. We propose \textbf{unrolling loss} for better performance, as
{
\begin{align}
    \cL_{\mathrm{Unrolling}}&=\lambda'||\bx_K-\bx_\mathrm{label}||_2^2
    \notag
    \\
    +\sum_{k=0}^{K-1}&~\mathbb{E}_{\epsilon\sim\mathcal{N}(0,\sigma^2I)}||\cD(\bm{\theta}; \bx_k+\epsilon)-\cD(\bm{\theta}; \bx_\mathrm{label})||^2_2
    \label{eq: unrolling loss}
\end{align}
}%
where $\bx_K$ is the output of the $K$-th and the final unrolling step, \textit{i.e.} the final reconstructed image, $\bx_\mathrm{label}$ is the ground truth image. Inspired by TRADES \cite{zhang2019theoretically}, our \textbf{unrolling loss} contains a robustness regularizer besides a residual norm for accuracy, and a hyper-parameter $\lambda'$ is introduced to balance the trade-off between accuracy and robustness. When $\lambda'=0$, the \textbf{unrolling loss} exploits the full potential of our {\us} architecture towards robustness; when $\lambda'$ approaches $+\infty$, the \textbf{unrolling loss} penalties the model's inaccuracy directly. The expectation here is, again, estimated through the Monte Carlo sampling using the same noises as the forwarding propagation.

Moreover, we do not only rely on \textbf{unrolling loss} to train {\us}. In general, we adopt MSE + Unrolling Stab scheme following MSE + Stab scheme in denoised smoothing \cite{salman2020denoised}. First, the denoiser is pre-trained on the ground truth image to remove added Gaussian noises. We use an MSE loss as denoised smoothing, but $\bx$ here is the ground truth image.
This pre-training only takes a small amount of time compared to the following fine-tuning. However, the pre-training can find a good starting point for fine-tuning, which leads to remarkably higher robustness of the final model.
Then, the denoiser is fine-tuned through a stability loss. Conventionally, an end-to-end (E2E) stability loss is used, as
\begin{equation}
    \cL_{\mathrm{E2E}} = ~\mathbb{E}_{\epsilon\sim\mathcal{N}(0,\sigma^2I)}||f(\bm{\theta}; \bx, \epsilon) - f_\mathrm{base}(\bx)||_2^2%,\quad\epsilon\sim\mathcal{N}(0, \sigma I^2)
\end{equation}
where $f$ is the smoothed model, including \ref{eq: denoised smoothing mri}, and $f_\mathrm{base}$ is the base model, \textit{i.e.} the trained vanilla {\modl}. However, we adopt \textbf{unrolling loss} for fine-tuning. We study the effectiveness of our training scheme in Sec. \ref{sec: experiment}.

% We, instead, adopt an unrolling form of stability loss to exploit the unrolling architecture of {\us}, which we call \textit{unrolling loss}, as
% \begin{align}
%     \cL_{\mathrm{Unrolling}}&=\lambda'||\bx_K-\bx_\mathrm{label}||_2^2
%     \notag
%     \\
%     +\sum_{k=0}^{K-1}&~\mathbb{E}_{\epsilon\sim\mathcal{N}(0,\sigma^2I)}||\cD(\bm{\theta}; \bx_k+\epsilon)-\cD(\bm{\theta}; \bx_\mathrm{label})||^2_2
%     \label{eq: unrolling loss}
% \end{align}
% where $\bx_K$ is the output of the $K$-th and the final unrolling step, \textit{i.e.} the final reconstructed image, $\bx_\mathrm{label}$ is the ground truth image. Inspired by TRADES \cite{zhang2019theoretically}, our unrolling loss contains a robustness regularizer besides one for accuracy in our unrolling loss, and $\lambda'$ is a hyper-parameter that balances the trade-off between accuracy and robustness. When $\lambda'=0$, the unrolling loss exploits the full potential of our {\us} architecture towards robustness; when $\lambda'$ approaches $+\infty$, the unrolling loss penalties the model's inaccuracy directly. The expectation here is, again, estimated through the Monte Carlo sampling using the same noises as the forwarding propagation.

We emphasize that $\cD(\bm{\theta}; \bx_\mathrm{label})$ in the unrolling loss as the reference image is carefully selected. Because of the convergence and added Gaussian noises, the denoiser $\cD(\cdot)$ and its input image $\bx_n + \epsilon$ are both unstable in the training process. Consequently, the choice for the reference image in the unrolling loss is significant.
We select $\cD(\bm{\theta};\bx_\mathrm{label})$ as the reference image, in which $\cD(\cdot)$ countacts the instability of the denoiser, and $\bx_\mathrm{label}$ makes the training more aggressive, promoting training efficiency.

% \vspace{-3mm}


==> sections_old/sec_preliminaries.tex <==
\section{Preliminaries and Problem Statement}
\label{sec: preliminaries}

In this section, we provide a brief background on MRI reconstruction and randomized smoothing. We will then motivate the lack of robustness   of MRI reconstruction and the problem of our interest. 


\vspace*{1mm}
\noindent \textbf{Setup of MRI reconstruction.} MRI reconstruction is an 
 ill-posed inverse problem \cite{compress}, which aims to reconstruct the original signal from its sparse observations. 
 In the context of multi-coil MRI reconstruction, let $\bx\in\mathbb{C}^{q}$ and $\mathbf y_c \in  \mathbb{C}^p$ (with $p < q$) denote the image to be recovered and its measurements associated with the $c$th  magnetic coil. We can cast the problem of MRI reconstruction  as 
%  can be described roughly as a model-fitting method to reconstruct   image with a data-consistency term. This is typically accomplished by adding a regularization term that enforces the sparsity-inducing prior on $\by$.
% The regularizer imposes additional constraints on the desired type of solution, resulting in an eventual solution that is more stable. 
% For multi-coil MRI reconstruction of an image 
% $\bx\in\mathbb{C}^{q}$, the optimization problem can be mathematically framed as
{
%\vspace*{-3mm}
\begin{align}
    \hat{\bx}=\underset{\bx}{\arg\min} ~\sum_{c=1}^{N_c}\|A_c \bx - \by_c \|^{2}_2 + \lambda \mathcal{R}(\bx),
    \label{eq:inv_pro}
\end{align}
}%
where $ N_c$ is the number of magnetic coils, $\mathcal{R}(\cdot)$ is a regularization function (\textit{e.g.}, $\ell_1$ norm to impose a sparse prior), and $\lambda > 0$ is a regularization parameter.  
In \eqref{eq:inv_pro},  $A_c = M \mathcal{F} S_c$ denotes   the forward system   operation,
where $M \in \{0,1\}^{p\times q}$ is a given sampling mask, 
$\mathcal{F}\in \mathbb{C}^{q\times q}$ is 
the $2D$ Fourier transformation, and $S_c \in 
\mathbb{C}^{q\times q}$ is a complex-valued position-dependent sensitivity map. 

% And the   regularizer $\mathcal{R}(\cdot)$  in \eqref{eq:inv_pro} is used to restrict the 
% solutions to the space of desirable
% images, and $\lambda$ is the regularization parameter controlling the trade-off between the residual norm and regularity.

% Choices for the regularizer in MRI reconstruction can vary from the $\ell_1$ penalty on wavelet coefficients~\cite{wave} or the most widely used CS method is total variation~\cite{totalv} denoising which enforces piecewise constant images by uniformly penalizing image gradients.

\subsection{MoDL and  the lack of robustness}
\label{sec: modl}


{\modl} relies on a formulation similar to \eqref{eq:inv_pro}, where the hand-crafted image regularization penalties in \eqref{eq:inv_pro} are replaced with learned priors. {\modl} has 
shown promise for MRI reconstruction
by combining a denoising network with a data-consistency ($\mathcal{DC}$) module in each stage
\cite{aggarwal2018modl}.
In the {\modl} model, Problem~\eqref{eq:inv_pro} is following:
    
{
\vspace*{-3mm}
\begin{align}
    \hat{\bx}=\underset{\bx}{\arg\min} ~  \sum_{c=1}^{N_c} \|A_c \bx - \by_c\|_2^2 + \lambda \| \bx - \cD (\bm{\theta};\bx) \|_2^2,
\label{eq:altmin}    
\end{align}
}%
%where $\nu \geq 0$ weights the data-fidelity term and $\mu \geq 0$ weights the proximity of $x$ to $z$ above. 
The problem can be solved by alternating between updating $\bx$ and $\cD (\bm{\theta};\bx)$.
The {\modl} scheme performs the update of $\bx$ (\textit{i.e.}, $\mathcal{DC}$) by Conjugate Gradient descent, and the update of $\cD (\bm{\theta};\bx)$ involving with a CNN denoiser ($\cD (\cdot)$) that is applied to the updated $\bx$.


\SL{[This is an important part to motivate our work. You need to define adversarial perturbations, undersampling rates, and unrolling steps, and associate them with math notations.]}
{\modl} is unstable against adversarial perturbations, different undersampling rates
% (When the sampling factor equals four,it will only collect $8\%$ of central k-space lines)
, and different unrolling steps
% ( $k$ for the number of alternative step between CNN denoiser update and Data consistence update) 
with training setup. 
The adversarial perturbation refers to a small, almost invisible to naked eyes, perturbation $\delta$ added to the input image $\bx_0$, which is constructed to deteriorate the performance of the model, as
\begin{equation}
    % \delta=\underset{\delta\sim\mathcal{S}}{\arg\max}~\cL(f(\bx+\delta), f(\bx))
    \underset{||\delta||_\infty\le r}{\arg\max}~\cL(f(\bx_0+\delta), f(\bx_0))
\end{equation}
% where $\mathcal{S}$ refers to a certain sphere around the data point $\bx$ with some distance measure.
where $f$ is the reconstruction model, and $r$ is the distance measure of the perturbation. Different undersampling rates refer to 
the new undersampling mask $M$ with different density is used to obtain the k-space measurements $\mathbf{y}_c$ from the ground truth in \eqref{eq:altmin} in the evaluation stage. And different unrolling steps mean a different number of iterations is used to solve \eqref{eq:altmin} in the evaluation stage.
In Fig. \ref{fig: weakness}, the reconstructed images blurs when adversarial perturbations are added to the undersampled input, a denser undersampling mask is used, and a larger number of unrolling steps is adopted in {\modl}.
 
\begin{figure}[htb]
%\vspace*{-3mm}
%    \centering
%    \begin{subfigure}{.10\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{Figures/output_vanilla_vis.pdf}
%        \caption{\footnotesize{clean data
%        }}
%    \end{subfigure}
%    \begin{subfigure}{.10\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{Figures/visualization/vanilla_MoDL_eps0.5_255.pdf}
%        \caption{\footnotesize{adversarial perturbations
%        }}
%    \end{subfigure}
%    \begin{subfigure}{.10\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{Figures/undersampling_vis.pdf}
%        \caption{\footnotesize{undersampling rate}}
%    \end{subfigure}
%    \begin{subfigure}{.10\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{Figures/unrolling_steps_vis.pdf}
%        \caption{\footnotesize{number of unrolling steps
%        }}
%    \end{subfigure}
    
%    \vspace*{-1em}
%    \caption{\footnotesize{{\modl}'s %instabiliites \textit{w.r.t.} adversarial perturbations, undersampling rate and number of unrolling steps}}
%    \label{fig: weakness}
%    \vspace*{-2mm}
\begin{tabular}[b]{cccc}
        \includegraphics[width=.2\linewidth, trim=70 10 70 10]{Figures/visualization/vanilla_MoDL_recon.pdf}
        &
        \includegraphics[width=.2\linewidth, trim=70 10 70 10]{Figures/visualization/vanilla_MoDL_eps0.5_255.pdf}
        &
        \includegraphics[width=.2\linewidth, trim=70 10 70 10]{Figures/visualization/undersampling_2.0_vis.pdf}
        &
        \includegraphics[width=.2\linewidth, trim=70 10 70 10]{Figures/visualization/unrolling_steps_16_clean_vis.pdf}
        \\[-0pt]
        \scriptsize{(a)} 
        & 
        \scriptsize{(b)} 
        &  
        \scriptsize{(c)} 
        &
        \scriptsize{(d)}

\end{tabular}
\vspace*{-5mm}
\caption{\footnotesize{{\modl}'s instabilities against adversarial perturbations, different undersampling rates, and different unrolling steps. (a) the reconstruction image from the clean image, (b) the reconstruction image from the adversarial perturbed image with the perturbation $||\delta||_{\infty}\le0.002$, (c) the reconstruction image when evaluated using a mask with the undersampling rate being 2 \hui{50\%?} (4 \hui{25\%?} in training), (d) the reconstruction image when evaluated using 16 unrolling steps (8 in training).}}
\label{fig: weakness}
\vspace*{-4.5mm}
\end{figure}

\subsection{Randomized smoothing} %and denoised smoothing}


Randomized smoothing \cite{cohen2019certified} uses a model's 
\SL{[why just classifier? makes it more general.]}
robustness to random noise to create a new model robust to adversarial perturbations. In classfication case, given a base classifier mapping from image domain $\mathbb R^d$ to classes $\mathcal Y$, the smoothed classifier $g$ 
%Given the CNN network by augmenting the data with noise ${x_{aliased}^{i},y^{i}}$
%\begin{equation}
%    f_{rs} = \frac{1}{K} \sum_{k=1}^{K} 
%    f_{\theta_{\text{noise}}}(x+\epsilon^{k}),\quad \epsilon\sim\mathcal N(0, \sigma^2I)
%\end{equation}
 returns the label which the base classifier $f$ is most likely to return when image $\bx$ is perturbed by Gaussian noise, as
is
{
\begin{align}
    g(\bx)=\underset{c\in\mathcal Y}{\arg\max}~ \mathbb P(f(\bx+\epsilon)=c),\quad \epsilon\sim\mathcal N(0, \sigma^2I)
    \label{eq: randomized smoothing}
\end{align}
}%
where the base classifier $f$ is trained with Gaussian noise augmented data, and Monte Carlo sampling is used to estimate the probability.

% Proved by Neyman-Pearson lemma, the smoothed classifier $g$ is certified to be robust to adversarial perturbations within a small $l_2$ radius compared to $\sigma$. This $l_2$ radius is related with the robustness of base classifier $f$ towards Gaussian noise. Consequently, in randomized smoothing, the base classifier is trained with Gaussian noise augmented data.

To avoid retraining the off-the-shelf model with Gaussian noise augmented data, paper \cite{salman2020denoised} proposed Denoised Smoothing where a denoiser $\cD (\cdot)$ is appended to the classifier $f$ to form a new base classifier $f \circ \cD$ robust to Gaussian noise. Then the smoothed classifier takes the majority vote over $f \circ \cD$, as
{
\begin{align}
    g(\bx)=\underset{c\in\mathcal Y}{\arg\max}~ \mathbb P(f(\cD (\bm{\theta};\bx + \epsilon))=c),\quad \epsilon\sim\mathcal N(0, \sigma^2I)
    \label{eq: denoised smoothing}
\end{align}
}

Noting that \eqref{eq: randomized smoothing} and \eqref{eq: denoised smoothing} cannot be directly used in MRI reconstruction tasks due to their regression-based learning objective, we convert \eqref{eq: denoised smoothing} into 
{
\begin{align}
    g(\bx)=\mathbb{E}_{\epsilon\sim\mathcal{N}(0, \sigma^2I)} f(\cD (\bm{\theta};\bx + \epsilon))
    \label{eq: denoised smoothing mri}
\end{align}
}
to get the smooth prediction.
%In denoised smoothing, the classifier $f$ is trained on clean data, and no data augmentation is needed. However, the denoiser $\cD (\cdot)$ is custom-trained to remove the Gaussian noise. They proposed two training objectives, mean square error (MSE) and stability (Stab). The latter takes the downstream classification task into account compared to the traditional MSE one. These two losses are defined as
%{\begin{align}
%    \cL_\mathrm{MSE}&=\mathbb{E}_{\epsilon\sim\mathcal N(0, \sigma^2I)}||\cD(\bm{\theta};\bx+\epsilon)-\bx||_2^2
%    \label{eq: MSE loss}
%    \\
%    \cL_\mathrm{Stab}&=\mathbb{E}_{\epsilon\sim\mathcal N(0, \sigma^2I)}||f(\cD(\bm{\theta};\bx+\epsilon))-f(\bx)||_2^2
    \label{eq: Stab loss}
%\end{align}}%

%MSE + Stab training scheme is used in denoised smoothing for efficiency and accuracy.

\SL{[why do we need to mention denoised smoothing? I did not get the point.]}
